FFaceNeRF: Few-shot Face Editing in Neural Radiance Fields

Recent 3D face editing methods using masks have produced high-quality edited images by leveraging Neural Radiance Fields (NeRF). Despite their impressive performance, existing methods often provide limited user control due to the use of pre-trained segmentation masks. To utilize masks with a desired layout, an extensive training dataset is required, which is challenging to gather. We present FFaceNeRF, a NeRF-based face editing technique that can overcome the challenge of limited user control due to the use of fixed mask layouts. Our method employs a geometry adapter with feature injection, allowing for effective manipulation of geometry attributes. Additionally, we adopt latent mixing for tri-plane augmentation, which enables training with a few samples. This facilitates rapid model adaptation to desired mask layouts, crucial for applications in fields like personalized medical imaging or creative face editing. Our comparative evaluations demonstrate that FFaceNeRF surpasses existing mask based face editing methods in terms of flexibility, control, and generated image quality, paving the way for future advancements in customized and high-fidelity 3D face editing. The code is available on the {\href{https://kwanyun.github.io/FFaceNeRF_page/}{project-page}}.

==> figures_tex/4_09_scaling.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/pfnerf_scaling2.png}
  \vspace{-5mm}
  \caption{Number of data used for training and resulting mIoU values. The mIoU value increases as the number of training data used becomes larger. }
  \label{fig:fig_scaling}
\end{figure}





==> figures_tex/90_others.tex <==
\input{figures_tex/9_03_augfeat}

==> figures_tex/x_app.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/X_facenerf_app.jpg}
  \vspace{-5mm}
  \caption{Visualization of partial style transfer.}\label{fig:x_app}
\end{figure*}


==> figures_tex/x_app2.tex <==
\begin{figure*}[h]
  \centering
  % the following command controls the width of the embedded PS file
  % (relative to the width of the current column)
  \includegraphics[width=\linewidth]{figures/x_ffacegan.png}
  \vspace{-5mm}
  \caption{Comparison of results produced by our FFaceGAN and the original DatasetGAN. This indicates effectiveness of our adapter and augmentation strategy.}\label{fig:x_app2}
\end{figure*}

==> figures_tex/x_aug.tex <==
\begin{figure}[t]
  \centering
  % the following command controls the width of the embedded PS file
  % (relative to the width of the current column)
  \includegraphics[width=\linewidth]{figures/x_ffacegan_aug.jpg}
  \caption{Visualization of augmentation results, which show color changes but preservation of the semantics of the source image.}\label{fig:x_aug}
\end{figure}

==> figures_tex/x_comparison.tex <==
\begin{figure*}[t]
  \centering
    \vspace{-3mm}
  \includegraphics[width=0.95\linewidth]{figures/x_comparison_final.png}
  \caption{Additional comparison results between our method, two baseline methods, and two additional methods. NeRFFaceEditing showed degraded quality with texture shifts and incomplete editing, particularly on elements like clothing. IDE-3D failed to reconstruct identity, FaceEdit3D failed to edit undefined regions, and InstructPix2NeRF exhibited limited control. In contrast, our method faithfully edited the source image in accordance with the target mask.}
  \label{fig:x_comp}
\vspace{-1mm}
\end{figure*}


==> figures_tex/x_faceedit.tex <==
\begin{figure}[t]
  \centering
  % the following command controls the width of the embedded PS file
  % (relative to the width of the current column)
  \includegraphics[width=0.8\linewidth]{figures/x_FaceEdit.png}
  \caption{Gaze direction editing results of FaceEdit3D.}
  \label{fig:x_faceedit}
  \vspace{-3mm}
\end{figure}



==> figures_tex/x_network.tex <==
\begin{figure}[h]
  \centering
  % the following command controls the width of the embedded PS file
  % (relative to the width of the current column)
  \hspace{-6mm}
  \includegraphics[width=1.05\linewidth]{figures/x_attention.png}
  \vspace{1mm}
  \caption{Visualization of our MLP network and multi-head self-attention network which are used as the geometry adapter.}\label{fig:network}
\end{figure}

==> figures_tex/x_ours.tex <==
\begin{figure*}[!t]
  \centering
  \vspace{3mm}
  \hspace{-7mm}
  \includegraphics[width=1.05\linewidth]{figures/X_ours.png}

  \caption{Additional results of FFaceNeRF in multi-view.}\label{fig:x_ours}
  
\end{figure*}

==> figures_tex/x_sketchface.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/x_sketchface.png}
   \vspace{-2mm}
   \caption{Gaze direction editing results of SketchFaceNeRF. Left shows source image and corresponding sketch, while right shows edited sketch and corresponding output face.}
   \label{fig:sketchface}
   \vspace{-1mm}
\end{figure}

==> figures_tex/x_statistical_result.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/results2.png}
   \vspace{-2mm}
   \caption{User study analysis results.}
   \label{fig:statistic}
   \vspace{-1mm}
\end{figure}

==> tables_tex/top_layer_list.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{3mm}
\caption{\fixq{List of the top 6 layers from the left in mIoU and L1, respectively}} %{-10pt}
\small
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
mIoU & 13 & 14 & 11 & 12 & 10 & 9 \\ \hline
L1 & 5 & 1 & 2 & 4 & 3 & 6 \\
\hline
\end{tabular}
\vspace{-5px}
\label{tab:top6_layers}
\end{table}
